Accountable AI Delegation in Banking: Identity, Commitment Controls, Decision Evidence and Recovery

An AI-assisted payment can pass assessment and lose release authority before commitment. We specify a banking delegation contract that checks current authority, the shared payment cap and the capacity of eligible instruments to cover losses. It books the new payment and its recovery demands and writes the outcome record in the same atomic transition. A paired example identifies the authorised mandate, applied rule and selection inputs a reviewer needs to assess mandate conformance. We show that, under fixed resource inputs, the transition preserves the payment cap and recovery feasibility when commitments and effective withdrawals are ordered against the same authoritative state. Reversing a transmitted priority changes the selected route in 4 of 32 distinct behavioural combinations, represented by 96 of 576 labelled contexts. The executor follows the transmitted rule in all of them. Reusing earlier state admits 23 releases in 123 histories blocked by the reference. Pooling recovery capacity admits 69 infeasible configurations in a grid of 576. Both current-state implementations agree with the reference in all 144 commitment histories and 624 concurrent schedules. The retention test recovers five specified outcome fields from each of 47 complete records. Fifteen survey responses informed requirements for resolving holds and handling uncertain delivery. An insurance example illustrates referral after an adverse coverage finding.

==> 1-journal-meta.tex <==
\renewcommand{\swJournalName}{Swissi AI Journal}
\renewcommand{\swISSNPrefix}{3043}
\renewcommand{\swISSNSuffix}{1921}
\renewcommand{\swJournalURL}{https://journal.swissi-ai.institute}
\renewcommand{\swJournalEmail}{journal@swissi-ai.institute}
\renewcommand{\swPublisher}{Swissi AI Journal}

\renewcommand{\swVolume}{2026}
\renewcommand{\swYear}{2026}
\renewcommand{\swDOI}{10.5281/zenodo.24394901}

\renewcommand{\swSwissiHash}{zn4e75rolmks}
\renewcommand{\swSwissiAddress}{Sw2:academic01:obj:p1:zn4e75rolmks26tnoxknvok6ayx332dnyqeiarfay5uhyqz2vbxa:fb76149f}

\renewcommand{\swArticleType}{\swLangText{Research Article}{Forschungsartikel}}

\renewcommand{\swLicence}{CC BY 4.0}
\renewcommand{\swLicenceURL}{https://creativecommons.org/licenses/by/4.0/}

\renewcommand{\swOpenAccessPolicyURL}{https://journal.swissi-ai.institute/authors\#open-access}
\renewcommand{\swCreditTaxonomyURL}{https://journal.swissi-ai.institute/authors\#credit-taxonomy}


==> 1-system/1-journal-meta.tex <==
\renewcommand{\swJournalName}{Swissi AI Journal}
\renewcommand{\swISSNPrefix}{3043}
\renewcommand{\swISSNSuffix}{1921}
\renewcommand{\swJournalURL}{https://journal.swissi-ai.institute}
\renewcommand{\swJournalEmail}{journal@swissi-ai.institute}
\renewcommand{\swPublisher}{Swissi AI Journal}

\renewcommand{\swVolume}{2026}
\renewcommand{\swYear}{2026}
\renewcommand{\swDOI}{10.5281/zenodo.24394901}

\renewcommand{\swSwissiHash}{zn4e75rolmks}
\renewcommand{\swSwissiAddress}{Sw2:academic01:obj:p1:zn4e75rolmks26tnoxknvok6ayx332dnyqeiarfay5uhyqz2vbxa:fb76149f}

\renewcommand{\swArticleType}{\swLangText{Research Article}{Forschungsartikel}}

\renewcommand{\swLicence}{CC BY 4.0}
\renewcommand{\swLicenceURL}{https://creativecommons.org/licenses/by/4.0/}

\renewcommand{\swOpenAccessPolicyURL}{https://journal.swissi-ai.institute/authors\#open-access}
\renewcommand{\swCreditTaxonomyURL}{https://journal.swissi-ai.institute/authors\#credit-taxonomy}

